Problems with Cosine as a Measure of Embedding Similarity for High Frequency Words

Cosine similarity of contextual embeddings is used in many NLP tasks (e.g., QA, IR, MT) and metrics (e.g., BERTScore). Here, we uncover systematic ways in which word similarities estimated by cosine over BERT embeddings are understated and trace this effect to training data frequency. We find that relative to human judgements, cosine similarity underestimates the similarity of frequent words with other instances of the same word or other words across contexts, even after controlling for polysemy and other factors. We conjecture that this underestimation of similarity for high frequency words is due to differences in the representational geometry of high and low frequency words and provide a formal argument for the two-dimensional case.

==> Sections/3RelatedWork.tex <==
\section{Related Work}
The impact of frequency on accuracy and reliability has mostly been studied on \textit{static} word embeddings like word2vec.
%For example,  \citeauthor {NIPS2014_feab05aa} shows how SGNS is implicit matrix factorization of word co-occurrences. 
Low frequency words have low reliability in neighbor judgements
\citep{hellrich-hahn-2016-bad}, and yield smaller inner products (cosines) \citep{mimno-thompson-2017-strange}, and higher frequency words have larger norms \cite{} [{\color{red}better to say low freq words have smaller norms}]. Frequency also correlates with stability (overlap in nearest neighbors) \citep{wendlandt-etal-2018-factors}, and plays a role in word analogies and bias \cite{NIPS2016_a486cd07, Caliskan183, zhao-etal-2018-gender}. 

Similar effects have been found in contextual embeddings, particularly for low-frequency senses, which seem to cause difficulties in WSD performance  for BERT and RoBERTA \citep{postma-etal-2016-always, blevins-zettlemoyer-2020-moving, gessler2021bert}. 
%Researchers also examine how frequency affects the syntactic rule learning find that model's performance on subject-verb agreement is heavily influenced by word frequency \cite{wei2021frequency}.
While previous work has thus mainly focused on reliability or stability of low frequency words or senses, our work focuses on the other end of the frequency range,  proposing that the BERT embedding representations of \textbf{high-frequency} words may also be problematic.  



% \cite{}.
% %notes

% BERT Has Uncommon Sense:Similarity Ranking for Word Sense BERTology
% Moving Down the Long Tail of Word Sense Disambiguation
% with Gloss Informed Bi-encoders

% Rare senses (but rare senses in polysemous, frequent words)

% Citation for:
% ~Patterns of Lexical Ambiguity in Contextualised Language Models

% " In line withour results, they reported polysemic senses to berated significantly more similar to one another inboth the human annotations and BERT Base em-beddings, and found a strong correlation betweenthe cosine distance of BERT sense centroids andaggregated relatedness judgements."

% Citation for our method:

% Moving Down the Long Tail of Word Sense Disambiguationwith Gloss Informed Bi-encoders


% "As suggested by Loureiro and Jorge (2019), we experimented with both the last hidden state and the sum of the lastfour hidden states as contextualised representation of a target word.7"

% "For both BERT models, summing over the last 4 hidden states improved correlation with the similarity ratings by about 6 points, and the correlation with the co-predication acceptability ratings by about 4 points. We will therefore report only results on this version in the remainder of this paper"

% For words that are tokenized into multiple subword pieces by the BERT tokenizer, we represent the word by the average representation of its subword pieces. 

%should we be training multiple models to see how these effects actually change

==> Sections/6Findings2.tex <==
\section{What is the effect of adding more data?}
It is challenging to replicate these results across various other models since it requires (in most cases) replicating the training data used for these models. We recommend that moving forward, models datasheets \cite{} are published with training data frequencies in order to help detect these frequency-based distortions.

\begin{table}[h!]
\centering
\begin{tabular}{|l|r|r|r|}
\hline
Freq & BERT & BERT-Large & BERT-ML \\ \hline
100-1k & X & X & X \\\hline
1k-10k & X & X & X \\\hline
10k-100k &  X & X & X \\\hline
100k-1m & X & X & X \\\hline
1m-10m & X & X & X \\\hline
10m+ & X & X & X \\\hline
\end{tabular}
\caption{Average radii of bounding hyperspheres of words of various frequency (based on BERT's original training data). We see how the sizes of these radii change across models with different training data.}
\end{table}

For now, we will rely on BERT's training data frequencies as a way to measure how these effects change across different training data. By examining how radii changes across BERT-Large and BERT-ML, we find that there are significant ways in which the geometric space occupied by words can change. This is an encouraging sign as it suggests that these distortions can be modified through different training data or methodologies. Future work should explore the impacts of training methodology changes as well as the impacts of fine-tuning.

% Our first experiments illustrate that lower frequency words have embeddings that can easily identify them, whereas higher frequency words are much more difficult to identify by their embeddings. Additionally, we find that the space occupied by a sibling cohort varies with the frequency of the word in its original training data.
%  \begin{subfigure}[b]{\columnwidth}
%      \centering
%      \includegraphics[width=\textwidth,height=4.8cm]{Images/Findings1/mistakesbywordfrequencyoffirsttoken.png}
%      \caption{}
%      \label{fig: frequency of first token}
%  \end{subfigure}

% We find that the performance of the identity probe degrades slightly when the word is tokenized into multiple parts and the first token maps to a non-word (a single or two characters, excluding words like “a”, and “i”). For example, the identity probe does slightly worse on words such as “bleach”, which is tokenized into “b”, “\#\#lea”, “\#\#ch”. The error rate of these words is 6\% compared to 2 - 4\% error rate across all other categories (see figure \ref{fig: frequency of first token}).


% \begin{figure}[ht]
%     \centering
%     \vspace{-0.5 em}
%      \includegraphics[width=.48\textwidth]{Images/Findings1/RadiusofBoundingBallvsWordFrequency.png}
%      \vspace{-1 em}
%      \caption{The radius of the minimal bounding ball of sibling embeddings of words is correlated with log(word frequency). Pearson's r: 0.63, \textit{p}  < .001}
%      \label{fig: radius vs word frequency}
%      \vspace{-0.5 em}
% \end{figure}

% We use a sentence-word pair for each target word and the # of sentences in the training data is the # of classes in the classifier. At test time, we use different sentence containing the target word, e.g. "The store was out of milk", and again use the vectors corresponding to "store" as input and ask the classifier to predict the identity of the word. The two embeddings of the "store" are sibling embeddings of each other --- .

% \footnote{Linear separability does not necessarily correlate with the size of the clusters. Imagine two sibling cohorts that are very far apart, the size of the cohorts would not necessarily correlate with their linear separability. Are more identifiable words more tightly clustered than less identifiable words? 
% }.
% ; the task here is trained to predict word identity just from the word's embedding.

% Each class is a word, and class selection for each model was random. This is very similar to the original masking task, except that instead of making predictions over the entire vocabulary, we simply classify words over 1000 classes. 
% and 2) how much does the word ’s identity impact its contextualized word embedding

